Towards Zero-shot Point Cloud Anomaly Detection: A Multi-View Projection Framework

Detecting anomalies within point clouds is crucial for various industrial applications, but traditional unsupervised methods face challenges due to data acquisition costs, early-stage production constraints, and limited generalization across product categories. To overcome these challenges, we introduce the Multi-View Projection (MVP) framework, leveraging pre-trained Vision-Language Models (VLMs) to detect anomalies. Specifically, MVP projects point cloud data into multi-view depth images, thereby translating point cloud anomaly detection into image anomaly detection. Following zero-shot image anomaly detection methods, pre-trained VLMs are utilized to detect anomalies on these depth images. Given that pre-trained VLMs are not inherently tailored for zero-shot point cloud anomaly detection and may lack specificity, we propose the integration of learnable visual and adaptive text prompting techniques to fine-tune these VLMs, thereby enhancing their detection performance. Extensive experiments on the MVTec 3D-AD and Real3D-AD demonstrate our proposed MVP framework's superior zero-shot anomaly detection performance and the prompting techniques' effectiveness. Real-world evaluations on automotive plastic part inspection further showcase that the proposed method can also be generalized to practical unseen scenarios. The code is available at https://github.com/hustCYQ/MVP-PCLIP.

==> Tables/scheme.tex <==

\begin{table}[thb]
    \centering

    \caption{Comparison of different schemes.}
    \label{tab:scheme}
    \renewcommand{\arraystretch}{1.1}
    \setlength\tabcolsep{3.0pt}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{p{3.2cm}<{\centering} p{2.6cm}<{\centering} p{2.6cm}<{\centering}}
            \toprule[1.5pt]
            \multirow{1}{*}{Scheme}     & \multirow{1}{*}{Train Data} & \multirow{1}{*}{Test Data}  \\
            \hline
            Supervised          & $\{\mathcal{X}_{N'},\mathcal{X}_{Ab'}\}$  &    $\{\mathcal{X}_{N},\mathcal{X}_{Ab}\}$      \\
            Unsupervised        & $\{\mathcal{X}_{N'}\}$   &   $\{\mathcal{X}_{N},\mathcal{X}_{Ab}\}$     \\
            \hline
            Zero-shot           & $\{\mathcal{X}_{Au}\}$    &  $\{\mathcal{X}_{N},\mathcal{X}_{Ab}\}$     \\

            \bottomrule[1.5pt]
        \end{tabular}
    }
\end{table}

==> figures/backbone.tex <==
\begin{figure}[h!]
\centering\includegraphics[width=\linewidth]{figures/pic8.png}
\caption{The point-wise performance using different backbones.}%\vspace{-5mm}
\label{fig:backbone}
\end{figure}
